Single-Shot Panoptic Segmentation

We present a novel end-to-end single-shot method that segments countable object instances (things) as well as background regions (stuff) into a non-overlapping panoptic segmentation at almost video frame rate. Current state-of-the-art methods are far from reaching video frame rate and mostly rely on merging instance segmentation with semantic background segmentation, making them impractical to use in many applications such as robotics. Our approach relaxes this requirement by using an object detector but is still able to resolve inter- and intra-class overlaps to achieve a non-overlapping segmentation. On top of a shared encoder-decoder backbone, we utilize multiple branches for semantic segmentation, object detection, and instance center prediction. Finally, our panoptic head combines all outputs into a panoptic segmentation and can even handle conflicting predictions between branches as well as certain false predictions. Our network achieves 32.6% PQ on MS-COCO at 23.5 FPS, opening up panoptic segmentation to a broader field of applications.

==> tables/ablation-thresh.tex <==
% Preview source code for paragraph 0

\begin{tabular}{c||ccc}
\hline 
\textbf{COCO Panoptic} & \multicolumn{3}{c}{Panoptic Seg. (\%)}\tabularnewline
Threshold & \textbf{PQ} & PQ\textsuperscript{th} & PQ\textsuperscript{st}\tabularnewline
\hline 
\hline 
0.25 & 26.8 & 29.6 & \textbf{22.6}\tabularnewline
0.30 & 28.5 & 32.4 & \textbf{22.6}\tabularnewline
0.35 & 29.4 & 34.1 & 22.4\tabularnewline
0.40 & \textbf{29.9} & 34.8 & 22.3\tabularnewline
0.45 & 29.8 & \textbf{34.9} & 22.2\tabularnewline
0.50 & 29.3 & 34.1 & 22.0\tabularnewline
0.55 & 28.3 & 32.7 & 21.8\tabularnewline
\end{tabular}


==> tables/comparison-detailed-flat.tex <==
% Preview source code for paragraph 0

\begin{tabular}{c|c|c||ccc|ccc|ccc|c}
\hline 
\multicolumn{13}{c}{\textbf{COCO Panoptic}}\tabularnewline
\hline 
\multicolumn{3}{c||}{\textbf{Comparison, Single-Shot}} & \multicolumn{10}{c}{Panoptic Seg. (\%)}\tabularnewline
Name & Backbone & Input size & \textbf{PQ} & SQ & RQ & \textbf{PQ}\textsuperscript{th} & SQ\textsuperscript{th} & RQ\textsuperscript{th} & \textbf{PQ}\textsuperscript{st} & SQ\textsuperscript{st} & RQ\textsuperscript{st} & FPS\tabularnewline
\hline 
\hline 
DeeperLab & LWMNV2 & $321\times321$ & 18.0 & 71.3 & 23.6 & 26.9 & 73.9 & 34.6 & 17.2 & 70.5 & 22.6 & 26.6\tabularnewline
 DeeperLab & LWMNV2 & $641\times641$ & 24.5 & 73.2 & 31.5 & 26.9 & 73.9 & 34.6 & 20.9 & 72.5 & 26.9 & 13.7\tabularnewline
 DeeperLab & WMNV2 & $641\times641$ & 28.1 & 75.3 & 35.8 & 30.8 & 75.5 & 39.1 & 24.1 & 74.6 & 30.9 & 12.0\tabularnewline
 DeeperLab & Xception-71 & $641\times641$ & \textbf{34.3} & \textbf{77.1} & \textbf{43.1} & \textbf{37.5} & \textbf{77.5} & \textbf{46.8} & \textbf{29.6} & \textbf{76.4} & 37.4 & 8.4\tabularnewline
 \hline
 Ours (SF) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.1 & 73.5 & 41.6 & 34.3 & 73.6 & 44.5 & 28.8 & 73.6 & 37.4 & 23.3\tabularnewline
 Ours (HC) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.2 & 73.8 & 41.6 & 34.5 & 73.9 & 44.3 & 28.8 & 73.6 & 37.4 & 23.3\tabularnewline
 Ours (CC) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.6 & 74.3 & 42.0 & 35.0 & 74.8 & 44.8 & 29.0 & 73.6 & \textbf{37.7} & 21.8\tabularnewline
\end{tabular}


==> tables/comparison-detailed.tex <==
% Preview source code for paragraph 0

\begin{tabular}{c|c|c|c||ccc}
\hline 
\multicolumn{7}{c}{\textbf{COCO Panoptic}}\tabularnewline
\hline 
\multicolumn{4}{c||}{\textbf{Comparison, Single-Shot}} & \multicolumn{3}{c}{Panoptic Seg. (\%)}\tabularnewline
Subset & Name & Backbone & Input size & \textbf{PQ} & SQ & RQ\tabularnewline
\hline 
\hline 
\multirow{7}{*}{All} & DeeperLab & Light Wider MNV2 & $321\times321$ & 18.0 & 71.3 & 23.6\tabularnewline
 & DeeperLab & Light Wider MNV2 & $641\times641$ & 24.5 & 73.2 & 31.5\tabularnewline
 & DeeperLab & Wider MNV2 & $641\times641$ & 28.1 & 75.3 & 35.8\tabularnewline
 & DeeperLab & Xception-71 & $641\times641$ & \textbf{34.3} & \textbf{77.1} & \textbf{43.1}\tabularnewline\cline{2-7}
 & Ours (SF) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.1 & 73.5 & 41.6\tabularnewline
 & Ours (HC) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.2 & 73.8 & 41.6\tabularnewline
 & Ours (CC) & ResNet-50 & $576\times\left[576, 864\right]$ & 32.6 & 74.3 & 42.0\tabularnewline
\hline 
\hline 
\multirow{7}{*}{Things} & DeeperLab & Light Wider MNV2 & $321\times321$ & 18.5 & 71.8 & 24.3\tabularnewline
 & DeeperLab & Light Wider MNV2 & $641\times641$ & 26.9 & 73.9 & 34.6\tabularnewline
 & DeeperLab & Wider MNV2 & $641\times641$ & 30.8 & 75.5 & 39.1\tabularnewline
 & DeeperLab & Xception-71 & $641\times641$ & \textbf{37.5} & \textbf{77.5} & \textbf{46.8}\tabularnewline\cline{2-7}
 & Ours (SF) & ResNet-50 & $576\times\left[576, 864\right]$ & 34.3 & 73.6 & 44.5\tabularnewline
 & Ours (HC) & ResNet-50 & $576\times\left[576, 864\right]$ & 34.5 & 73.9 & 44.3\tabularnewline
 & Ours (CC) & ResNet-50 & $576\times\left[576, 864\right]$ & 35.0 & 74.8 & 44.8\tabularnewline
\hline 
\hline 
\multirow{7}{*}{Stuff} & DeeperLab & Light Wider MNV2 & $321\times321$ & 17.2 & 70.5 & 22.6\tabularnewline
 & DeeperLab & Light Wider MNV2 & $641\times641$ & 20.9 & 72.5 & 26.9\tabularnewline
 & DeeperLab & Wider MNV2 & $641\times641$ & 24.1 & 74.6 & 30.9\tabularnewline
 & DeeperLab & Xception-71 & $641\times641$ & \textbf{29.6} & \textbf{76.4} & 37.4\tabularnewline\cline{2-7}
 & Ours (SF) & ResNet-50 & $576\times\left[576, 864\right]$ & 28.8 & 73.6 & 37.4\tabularnewline
 & Ours (HC) & ResNet-50 & $576\times\left[576, 864\right]$ & 28.8 & 73.6 & 37.4\tabularnewline
 & Ours (CC) & ResNet-50 & $576\times\left[576, 864\right]$ & 29.0 & 73.6 & \textbf{37.7}\tabularnewline
\end{tabular}


==> tables/obj-det-mixed.tex <==
\begin{tabular}{c|c|c||ccc}
\hline 
\multicolumn{3}{c||}{\textbf{COCO Detection}} & \multicolumn{3}{c}{Object Det. (\%)}\tabularnewline
ResNet & Optimizer & Mixed LR & \textbf{AP} & AP\textsuperscript{50} & AP\textsuperscript{75}\tabularnewline
\hline 
\hline 
50 & Adam & - & 32.8 & 50.7 & 34.6\tabularnewline
50 & Adam & \checkmark & 33.1 & 51.1 & 34.7\tabularnewline
 &  &  & \textit{\footnotesize{}+0.3} & \textit{\footnotesize{}+0.4} & \textit{\footnotesize{}+0.1}\tabularnewline
\end{tabular}


==> tables/policy-ablation.tex <==
\begin{tabular}{c|c||ccc}
\hline 
\multicolumn{5}{c}{\textbf{COCO Panoptic}}\tabularnewline
\hline 
\multicolumn{2}{c||}{\textbf{Results, 1-stage}} & \multicolumn{3}{c}{Panoptic Seg. (\%)}\tabularnewline
Name & Policy & \textbf{PQ} & PQ\textsuperscript{th} & PQ\textsuperscript{st}\tabularnewline
\hline 
\hline 
Ours & Smallest First & 29.3 & 33.8 & \textbf{22.5}\tabularnewline
Ours & Highest Confidence & 29.6 & 34.2 & \textbf{22.5}\tabularnewline
Ours & Closest Center & \textbf{29.9} & \textbf{34.8} & 22.3\tabularnewline
\end{tabular}


==> tables/results-inst-center.tex <==
\begin{tabular}{c|c||c|c}
\hline 
\multicolumn{2}{c||}{\textbf{COCO Panoptic}} & \multicolumn{2}{c}{Instance Center Prediction}\tabularnewline
Name & Backbone & \textbf{Correct (\%)} & Total Pixels\tabularnewline
\hline 
\hline 
Ours & ResNet-50 & 90.8 & 62.0M \tabularnewline
\end{tabular}


==> tables/results-retinanet.tex <==
\begin{tabular}{c|c||ccc}
\hline 
\multicolumn{2}{c||}{\textbf{COCO Detection}} & \multicolumn{3}{c}{Object Detection (\%)}\tabularnewline
Model & Size & \textbf{AP} & AP\textsuperscript{50} & AP\textsuperscript{75} \tabularnewline
\hline 
\hline 
Ours & 544 & 30.8 & 48.8 & 32.2 \tabularnewline
Ours & 640 & 33.1 & 51.1 & 34.7 \tabularnewline
\hline 
RetinaNet \cite{Lin_17_ICCV} & 400 & 30.5 & 47.8 & 32.7 \tabularnewline
RetinaNet \cite{Lin_17_ICCV} & 600 & 34.3 & 53.2 & 36.9 \tabularnewline
RetinaNet \cite{Lin_17_ICCV} & 800 & \textbf{35.7} & \textbf{55.0} & \textbf{38.5} \tabularnewline
\end{tabular}


==> tables/results-sem-seg.tex <==
\begin{tabular}{c|c||c}
\hline 
\multicolumn{2}{c||}{\textbf{COCO Stuff}} & \multicolumn{1}{c}{Semantic Segm. (\%)}\tabularnewline
Name & Backbone & \textbf{mIoU}\tabularnewline
\hline 
\hline 
Ours & ResNet-50 & 26.9\tabularnewline
Ours & ResNet-101 & 27.9\tabularnewline
\hline 
Sem. FPN$^{\dag}$ \cite{Kirillov_19_CVPR_PanFPN} & ResNeXt-152 & 27.8\tabularnewline
\end{tabular}


==> tables/two_branches_segdet_with_pq_sf.tex <==
\begin{tabular}{c|c||ccc|c|c}
\hline 
\multicolumn{7}{c}{\textbf{COCO Panoptic}}\tabularnewline
\hline 
\multicolumn{2}{c||}{Weights} & \multicolumn{3}{c|}{Pan. Seg.} & Seg. & Det.\tabularnewline
Sem. & Obj. & \textbf{PQ} & PQ\textsuperscript{th} & PQ\textsuperscript{st} & mIoU & AP\tabularnewline
\hline
\hline
1.00 & - & - & - & - & \textbf{50.0} & - \tabularnewline
- & 1.00 & - & - & - & - & \textbf{31.2} \tabularnewline
\hline
0.20 & 0.80 & 28.7 & 33.8 & 21.1 & 48.4 & \textbf{30.5}\tabularnewline
0.25 & 0.75 & 29.1 & 34.0 & 21.7 & 49.0 & \textbf{30.5}\tabularnewline
0.33 & 0.66 & \textbf{29.3} & \textbf{34.3} & 21.9 & 49.6 & 30.2\tabularnewline
\textbf{0.50} & \textbf{0.50} & \textbf{29.3} & 33.8 & 22.5 & 50.2 & 29.2\tabularnewline
0.66 & 0.33 & 29.2 & 33.2 & \textit{23.0} & \textbf{50.4} & 27.7\tabularnewline
0.75 & 0.25 & 28.6 & 32.3 & 22.9 & 50.2 & 26.7\tabularnewline
0.80 & 0.20 & 28.2 & 31.7 & 22.8 & 50.2 & 25.9\tabularnewline
\end{tabular}

